Learning-based MPC from Big Data Using Reinforcement Learning

This paper presents an approach for learning Model Predictive Control (MPC) schemes directly from data using Reinforcement Learning (RL) methods. The state-of-the-art learning methods use RL to improve the performance of parameterized MPC schemes. However, these learning algorithms are often gradient-based methods that require frequent evaluations of computationally expensive MPC schemes, thereby restricting their use on big datasets. We propose to tackle this issue by using tools from RL to learn a parameterized MPC scheme directly from data in an offline fashion. Our approach derives an MPC scheme without having to solve it over the collected dataset, thereby eliminating the computational complexity of existing techniques for big data. We evaluate the proposed method on three simulated experiments of varying complexity.

==> sections/background_old.tex <==
\section{Background}\label{sec:back}
% Model Predictive Control (parameterized)

\subsection{Parameterised MPC scheme}
We consider a real system described by a discrete MDP having a (possibly stochastic) state dynamics
\begin{align}
\mathbb{P}[s_+|s,a] \label{eq:tf1}
\end{align}
which represents the probability that executing action $a$ in state $s$ leading to state $s_+$. We label the stage cost associated to the MDP as $L(s,a)$
\begin{equation}
L(s,a)=l(s,a)+\mathcal{I}_\infty (h(s,a)) +\mathcal{I}_\infty (g(a)) 
\label{eq:st1}
\end{equation}
In \eqref{eq:st1}, function $l(s,a)$ captures cost associated to different state-action pairs, while the constraints $h(s,a)$ and $g(a)$ capture the undesirable state-action pairs. Note that \eqref{eq:tf1} is typically represented in the control literature as $s_+=f(s,a)$ where $f$ is a possibly nonlinear function. The indicator function $\mathcal{I}_\infty(x)$ penalizes constraint violations
\begin{equation}
\mathcal{I}_\infty(x) = \begin{cases}
\infty & \text{if}\ x > 0 \\
0 & \text{otherwise}
\end{cases} \nonumber
\end{equation} 
\eqref{eq:st1} assumes infinite value when constraints are violated. The underlying MDP with the associated stage cost $L$ and discount factor $0 \leq \gamma < 1$ is assumed to yield a well-posed problem.

\subsection{parameterized mpc}
We consider a model of the real system having a state transition dynamics
\begin{align}
\mathbb{P}[\hat{s}_+|s,a]\label{eq:tf2}
\end{align}
which typically do not match \eqref{eq:tf1}. \eqref{eq:tf2} trivially includes deterministic models and can also be given as $\hat{s}_+ = \hat{f}(s,a)$. A parameterized MPC scheme of horizon $N$ for such a system at a current state $s$ is
\begin{subequations}
\begin{align}
J(s) = \min_{u,x}&\quad \sum_{k=0}^{N-1} \gamma^k L_\theta(x_k,u_k) + \gamma^N V^f_\theta(x_N)  \\
\mathrm{s.t.}&\quad x_{k+1} = \hat{f}_\theta(x_k, u_k),\ x_0 = s  \\
&\quad h_\theta(x_k,u_k) \leq 0,\ h^f_\theta(x_N) \leq 0 \\
&\quad g(u_k) \leq 0
\end{align}\label{eq:mpc}
\end{subequations} 
\eqref{eq:mpc} holds stage a cost parameterization $L_\theta$, a terminal cost parameterization $V^f_\theta$, a constraint parameterization $h_\theta$, a terminal constraint parameterization $h_\theta^f$ and a model parameterization $f_\theta$. While pure action constraints $g(a) \leq 0$ are arguably fixed, mixed constraints $h_\theta(s,a)\leq 0$ are parameterized to capture the feasible state space regions in which $L_\theta$ is finite. $f_\theta(s, a)$ takes into account the uncerstain parameters and lump variables introduced for modelling the real system dynamics.

%In an MPC scheme, the stage cost often takes the form of a quadratic cost with diagonal terms. 
%
%Usually, a quadratic stage cost with diagonal terms is preferred for more explanable behaviour. The $\theta$ parameter for model can be learned with system identification methods from the system data (ref), while constraint parameterization is known a priori for the given system. Such constraints would take into account the actuator saturation, safety requirements present in the problem domain. 
%
%An important point to obersve is that, the classical way of formulating the MPC scheme does not tune for overall performance. Furthermore, it requires to use all the machinary to get parameter values. In recent times, RL methods have been used to further tune the MPC parameters (ref). However, such methods require solving MPC scheme while carrying out parameter updates, as discussed in following discussion. Additionally, the iterative way of updating may result in suboptimal parameters due to covariate data shift (ref) and may require access to the real system to correct for it. In many systems, such an access is expensive and also dangerous. In this work, we propose an alternate mechanism to tune MPC parameters from available system data. 

\subsection{MPC-based function approximation for MDPs}
Solving the underlying discrete MDP consists of finding an optimal \textit{policy}: a function $\pi$ that maps states $s$ into action $a$ for minimizing the cumulative cost $J$
\begin{align}
J(s, \pi) =\ \mathbb E\left [\left.\sum_{k=0}^\infty \gamma^k L(s_k,a_k)\,\right|\,s_0 = s, a_k=\pi(s_k)\right]
\end{align}
where $L(s,a)$ is the stage cost given in \eqref{eq:st1}. We label $\pi_*(s)$ the optimal policy, $Q_*(s,a)$ the action-value function, and $V_*(s)$ the value function. The policy and value functions are solution of the Bellman equations \citep{sutton2018reinforcement}:
\begin{align}
Q_*(s,a) &= L(s,a)+\gamma \mathbb{E}[V_*(s_+|s,a)] \nonumber\\
V_*(s) &= Q_*(s,\pi_*(s)) = \min_a Q_*(s,a) \nonumber
\end{align}
We briefly recall next the theory behind MPC-based approximations of these functions. \citep{gros2019data} consider a modified stage cost:
\begin{equation}
\hat{L}(s,a)=\begin{cases}
Q_*(s,a)-\gamma V^+(s,a) & \text{if}\ V^+(s,a) < \infty \\
\infty & \text{otherwise}
\end{cases} \label{eq:st2}%
\end{equation}
where $V^+(s,a)=\mathbb{E}[V_*(\hat{s}_+)|s,a]$ uses the expected value stemming from the model of system dynamics. 

\begin{theorem}\citep{gros2019data}\label{th:rlmpc}
Consider the optimal value function
\begin{align}
\hat{V}_N(s) = \min_\pi \mathbb{E} \big[ \gamma^N V_*(\hat{s}^\pi_N) + \sum_{k=0}^{N-1}\gamma^k \hat{L}(\hat{s}^\pi_k, \pi(\hat{s}^\pi_k)) \big]
\end{align}
associated to the stage cost \eqref{eq:st2}, the state transition model \eqref{eq:tf2}, and the terminal cost $V_*(s)$ over an optimization horizon $N$. Here we define $\hat{s}_{0,\dots,N}$ as the (possibly stochastic) trajectories of the state transition model $\mathbb{P}[\hat{s}_+|s,a]$ under a policy $\pi$, starting from $\hat{s}^\pi_0 = s$. We will label $\hat{\pi}$ as the optimal policy associated to $\hat{V}_N(s)$ and $\hat{Q}_N(s,a)$ the associated action-value functions. Consider the set $\mathcal{S}$ such that
\begin{align}
|\mathbb{E}[V_*(\hat{s}^{\pi_*}_k)]|<\infty,\quad \forall s\in \mathcal{S},\quad \forall k
\end{align}
The the following identities hold on $\mathcal{S}$.
\begin{itemize}
\item[i] $\hat{V}_N(s) = V_*(s)$
\item[ii] $\hat{\pi}(s) = \pi_*(s)$
\item[iii] $\hat{Q}_N(s,a) = Q_*(s,a)$ for the inputs $a$ such that $|\mathbb{E}[V_*(\hat{s}_+|s,a)]<\infty|$
\end{itemize}
\end{theorem}

Theorem \ref{th:rlmpc} states that, under some conditions, an MPC scheme using the model $\mathbb{P}[\hat{s}_+|s,a]$ and the modified stage cost \eqref{eq:st2} yields the optimal policy $\pi_*$ for the true MDP, together with the associated optimal value functions. Simply stated, an optimal policy can be generated using an MPC scheme based on simplified or inaccurate model dynamics provided that the MPC stage cost is adequately modified. In particular, an MPC scheme based on a deterministic model can yield the optimal policy and value functions of a stochastic MDP. \citep{gros2019data} suggests learning the stage cost modification $\hat{L}$ using RL tools oweing to the difficulty of evaluating \eqref{eq:st2}.

\subsection{MPC-based RL}
The MPC-based RL methods bypass evaluation of \eqref{eq:st2} by directly learning $\hat{L}$ from data. Hence, using the RL machinery, an MPC scheme can be learned in an iterative way, just like how weight of a policy approximated using a DNN are learned. Essentially, an MPC scheme would be used to carry approximations of the policy and value functions for an MDP. 

We consider the following parameterization of an MPC scheme for approximating the value function $V$ of a generic MDP:
\begin{subequations}
\begin{align}
V_{\theta}(s) = \min_{u,x,\sigma}&\quad \sum_{k=0}^{N-1} \gamma^k L_\theta(x_k,u_k) + w^T\sigma_k) \nonumber \\
&\quad + \gamma^N (V^f_\theta(x_N) + w_f^T\sigma_N) \label{eq:v1c0}\\
\mathrm{s.t.}&\quad x_{k+1} = f_\theta(x_k, u_k),\ x_0 = s \label{eq:v1c1} \\
&\quad h_\theta(x_k,u_k) \leq \sigma_k,\ h^f_\theta(x_N) \leq \sigma_N \label{eq:v1c2}\\
&\quad \sigma_k \geq 0, \ \sigma_N \geq 0 \label{eq:v1c3}\\
&\quad g(u_k) \leq 0 \label{eq:v1c4}
\end{align} \label{eq:v1}%
\end{subequations} 
\eqref{eq:v1} holds parameterization from \eqref{eq:mpc}. Additionally, an $l_1$ relaxation of the mixed constraints \eqref{eq:v1c4} is carried out using slack variables $\sigma_k$ to avoid infinite penalties in case of constraint violations. The corresponding policy is 
\begin{align}
\pi_\theta(s) = u^*_0 \label{eq:pi1}
\end{align}
where $u^*_0$ is the first element of the inpute sequence $u^*_0, \dots, u^*_{N-1}$ solution of \eqref{eq:v1} for a given state $s$. Similarly, the associated action-value function $Q$ approximation is
\begin{subequations}
\begin{align}
Q_{\theta}(s,a) = \min_{u,x,\sigma}&\quad \eqref{eq:v1c0} \\
\mathrm{s.t.}&\quad \eqref{eq:v1c1}-\eqref{eq:v1c4} \label{eq:q1c4} \\
&\quad u_0 = a \label{eq:q1c5} 
\end{align} \label{eq:q1}%
\end{subequations} 
For these value function approximations, the Bellman equations still hold:
\begin{align}
\pi_\theta(s) = \arg\min_a Q_\theta(s,a), 
\quad V_\theta(s) = \min_a Q_\theta(s,a) \nonumber
\end{align}
where $\pi_\theta(s)$ is the optimal policy for \eqref{eq:v1} and \eqref{eq:q1}.

In most RL methods, the optimal control policy required for solving the task at hand is learned either directly or indirectly. Indirect methods of finding the policy rely on learning an approximation of the optimal value function underlying the MDP, typically based on Temporal Difference methods \citep{kober2013reinforcement}. Direct RL methods seek to learn the policy directly with either stochastic or deterministic policy gradient methods \citep{silver2014deterministic}. However, such direct methods typically require finding an approximation of the value functions to compute the updates of the policy parameters. In both approaches, an MPC-based approximator can be plugged in with additional derivative definitions. When approximating $Q$ as in \eqref{eq:q1} for using temporal difference methods, like $Q$ learning \citep{watkins1992q}, the objective is to better approximate $Q_*$ with $Q_\theta$. 
\begin{align*}
\theta =& \arg\min_\theta \mathbb{E}_{\rho \sim s^\pi} \big[ (Q_*(s,a) - Q_\theta(s,a))^2 \big] 
\end{align*}
wherein, the expectation is taken over state distribution induced by the policy $\pi$. The iterative parameter update is
\begin{align}
\delta =&\ L(s,a) + \gamma V_\theta (s_+) - Q_\theta (s,a) \\
\theta \leftarrow &\ \theta + \alpha \mathbb{E} \big[\delta \nabla_\theta Q_\theta (s,a)\big] \label{eq:thup1}
\end{align}
For MPC-based approximation of state-action value function, the gradient of $Q_\theta$ is given by \citep{buskens2001sensitivity},
\begin{equation}
\nabla_\theta Q_\theta(s,a) = \nabla_\theta \mathcal{L}(s,y^*) \label{eq:gradq}
\end{equation}
wherein $y^*$ is the primal-dual solution of \eqref{eq:q1} and $\mathcal{L}$ is the associated Lagrange function. 

Most direct policy search methods make use of either policy gradient theorem \citep{sutton2000policy} pr deterministic policy gradient theorem \citep{silver2014deterministic}. Both approaches require an intermediate approximation of value function which is learned using temporal difference methods. additionally, for policy parameter update, we need gradient of policy with respect to parameter vector. For example, in case of deterministic policy gradient,  
\begin{align}
\theta \leftarrow &\ \theta + \alpha \mathbb{E} \big[\nabla_\theta \pi_\theta \nabla_\phi Q_\phi (s,a)\big] \label{eq:thup2}
\end{align}
wherein, MPC parameterized with $\theta$ is used to carry policy approximation asin \eqref{eq:pi1}, while $Q$ function is parameterized with $\phi$, typically with another approximator. The sensitivities of $\pi$ with respect to $\theta$ are given by \citep{buskens2001sensitivity} as,
\begin{align}
\nabla_\theta \pi_\theta(s) = - \nabla_\theta \xi_\theta(s,y^*)\nabla_y\xi_\theta(s,y^*)^{-1}\frac{\partial y}{\partial u_0}
\label{eq:gradpi}
\end{align}
where $y^*$ is the primal-dual solution and $\xi_\theta(s,y)$ gathers the primal-dual KKT conditions for \eqref{eq:v1}.


Using MPC-based RL methods, we can tune MPC scheme for better closed-loop performance. However, both approaches require solving the corresponding MPC scheme and evaluating sensitivities for update equations \eqref{eq:thup1} and \eqref{eq:thup2}. For tuning an MPC scheme using these update rules would require a lot computational expense. Additionally, classical RL methods operate in fundamentally \textit{online} learning paradigm and involve iteratively collecting experience by interacting with the system. In many tasks, such online interaction is impractical, either because data collection is expensive (e.g., in robotics, educational agents, or healthcare) and dangerous (e.g., in autonomous driving, or healthcare). Furthermore, even in domains where online interaction is feasible, we might still prefer to utilize previously collected data instead -- for example, if the domain is complex and effective generalization requires large datasets. many commonly used reinforcement learning methods can learn from off-policy data, but such methods often cannot learn effectively from entire offline data, without any additional on-policy interaction \citep{levine2020offline}. High-dimensional and expressive function approximation generally exacerbates this issue, since function approximation leaves the algorithms vulnerable to distributional shift, one of the central challenges with offline reinforcement learning. We propose an alternative to this by making using to the first take-way, by learning the modified stage cost directly from the available data. 



==> sections/challenges_with_big_data.tex <==
\section{Challenges with RL for MPC on big data} \label{sec:challenges}

Using MPC-based RL methods, we can tune MPC scheme for better closed-loop performance. However, both approaches require solving the corresponding MPC scheme and evaluating sensitivities for update equations \eqref{eq:thup1} and \eqref{eq:thup2}. For tuning an MPC scheme using these update rules would require a lot computational expense. Additionally, classical RL methods operate in fundamentally \textit{online} learning paradigm and involve iteratively collecting experience by interacting with the system. In many tasks, such online interaction is impractical, either because data collection is expensive (e.g., in robotics, educational agents, or healthcare) or it is dangerous (e.g., in autonomous driving, or healthcare). Furthermore, even in domains where online interaction is feasible, we might still prefer to utilize previously collected data instead -- for example, if the domain is complex and effective generalization requires large datasets. Many commonly used Reinforcement Learning methods can learn from off-policy data, but such methods often cannot learn effectively from entire offline data, without any additional on-policy interaction \citep{levine2020offline}. High-dimensional and expressive function approximation generally exacerbates this issue, since function approximation leaves the algorithms vulnerable to distributional shift, one of the central challenges with offline reinforcement learning. We propose an alternative to this by making using to the first take-way, by learning the modified stage cost directly from the available data. 

==> sections/introduction_old.tex <==
\section{Introduction}
%format: MPC and learning from big data -->(existing approaches on mpc and learning ) --> RL MPC --> how we do it 
% classic MPC intro
%introducing MPC and classical learning approach on MPC:
Real-life engineering applications with complex dynamics with constraints demand advanced control methods for safe and efficient operation. Model Predictive Control (MPC) is an advanced control method for working with complex multivariate dynamics and constraints, which is well suited for such applications. However, applying MPC to many applications faces challenges, such as the difficulty of modelling the system dynamics and achieving robust performance with low online computations and memory requirements. For a given optimization objective, MPC relies on some form of a model predicting the system dynamics to compute appropriate control actions. 
%designig mpc and challenges, systme identifiication cost tuning etc
%erecent data driven approaches and benefits

%conventional model learning approach and their drawbacks
Such models have often simplified representations of system dynamics with lump parameters to capture the input-output relations. Such models with lump parameters can be uncertain and need further tuning for close-loop performance improvement. System Identification methods and, recently, Machine learning tools have been used to identify these parameters using available data \citep{wu2019machine, lucia2018deep}. However, such approaches focus on better fitting the model to the data. This approach may not necessarily yield better closed-loop performance as the model adjustment here is not tied directly to the performance improvement.

%RLMPC approach
Gros et.al.~\cite{gros2019data} introduced RL for MPC in a holistic manner, by using MPC as a function approximator for the RL policy. This approach facilitates adjusting MPC parameters directly using RL to improve the control performance than relying only on the accuracy of the model. In a fully parameterized MPC formulation, RL can be used to adjust the model, cost, and constraints for improving the performance thereby providing larger flexibility in adapting the MPC formulation. Exploring this idea further, various works were published recently investigating MPC-based RL methods \cite{group papers on methods} and have been applied for different applications \cite{application papers}. 

% However, evaluating the MPC scheme for every state transition to learn from is super expensive.
These methods are more suitable for improving the MPC in an online setting by alternating between iteratively sampling and adapting the MPC. But applying these methods to formulate an MPC scheme offline can be cumbersome as it might need an enormous amount of MPC's to be computed depending on the data size and might require access to the system. This is a critical issue while trying to formulate an MPC scheme from big data which can be the case in many real-world applications. 

%our approach and advantages
In this paper, we propose an alternate approach to learning MPC formulation offline using available system data with RL tools. We make use of the modified stage cost suggested in \citep[Theorem 1]{gros2019data} by learning the required value function approximations from the data and learning the MPC formulation. We further illustrate this by learning stage cost and model on a simple linear system and further on the pendulum. 

The contributions of this paper are as follows:
\begin{itemize}
    \item ENabling to design/tune MPC from big data offline
    \item INtegrating it with the RLMPC framework with performance targeted tunging
\end{itemize}





%Introducing RL and RLMPC
%Reinforcement Learning (RL) is a powerful tool for solving Markov Decision Processes (MDPs) without depending on a priori knowledge of the underlying system dynamics. Most RL methods work with observed state transitions and stage cost realizations i.e. rewards for finding the close-to-optimal policy. In recent years, RL has gained popularity due to its accomplishments ranging from success in Atari games \citep{mnih2013playing} and in robotics \citep{heess2017emergence} to mastering the game of Go \citep{silver2016mastering}. 

%The issues with formulating MPC online and our spectacular solution :D 




%In most RL methods, the policy and required value functions associated with the underlying MDP are approximated with a generic function approximator, typically a deep neural network, and are learned while interacting with the system. Recently, \citep{gros2019data} proposed an MPC-based function approximator for generic MDPs and the approaches to tune its parameters through RL tools. An MPC-based policy and value function approximations offer a high explainability about the policy behaviour and are equipped with a broad set of theoretical tools for formal verification of the policy in terms of safety and stability. Exploiting this, various works have been proposed investigating MPC-based RL methods for different applications (ref). Such MPC-based RL methods can also be viewed as tuning MPC scheme using RL tools for better performance. Essentially, parameterizations and lump variables in stage cost and model dynamics are tuned for better close-loop performance, to better suit the task at hand.





The paper is structured as follows. Section \ref{sec:back} gives an overview of the MPC-based function approximators from \citep{gros2019data}. Section \ref{sec:method} details the proposed offline MPC learning scheme. Section \ref{sec:exp} discusses the experimental setup for pointmass and pendulum tasks, and the obtained results, followed by conclusion in section \ref{sec:con}. \\
